Sharp Periodic Flares and Long-Term Variability in the High-Mass X-ray Binary XTE J1829-098 from RXTE PCA, Swift BAT and MAXI Observations

XTE J1829-098 is a transient X-ray pulsar with a period of ~7.8 s. It is a candidate Be star system, although the evidence for this is not yet definitive. We investigated the twenty-year long X-ray light curve using the Rossi X-ray Timing Explorer Proportional Counter Array (PCA), Neil Gehrels Swift Observatory Burst Alert Telescope (BAT), and the Monitor of All-sky X-ray Image (MAXI). We find that all three light curves are clearly modulated on the ~244 day orbital period previously reported from PCA monitoring observations, with outbursts confined to a narrow phase range. The light curves also show that XTE J1829-098 was in an inactive state between approximately December 2008 and April 2018 and no strong outbursts occurred. Such behavior is typical of Be X-ray binary systems, with the absence of outbursts likely related to the dissipation of the Be star's decretion disk. The mean outburst shapes can be approximated with a triangular profile and, from a joint fit of this to all three light curves, we refine the orbital period to 243.95 +/- 0.04 days. The mean outburst profile does not show any asymmetry and has a total phase duration of 0.140 +/- 0.007. However, the PCA light curve shows that there is considerable cycle-to-cycle variability of the individual outbursts. We compare the properties of XTE J1829-098 with other sources that show short phase-duration outbursts, in particular GS 1843-02 (2S 1845-024) which has a very similar orbital period, but longer pulse period, and whose orbit is known to be highly eccentric.

==> 1829_figures.tex <==








==> 1829_tables.tex <==













% NOW INCORPORATED IN TABLE ABOVE (HOPEFULLY)
% pulse period measurements
%\clearpage
%\begin{deluxetable}{lccc}
%%\rotate
%\tablecolumns{8}
%\tabletypesize{\small}
%\tablewidth{0pc}
%\tablecaption{Pulse Period Measurements of \src}
%\tablehead{
%\colhead{Mission} & \colhead{Observation Time} & \colhead{Pulse Period} &\colhead{Ref.} \cr
%\\
%\colhead{}  & \colhead{(MJD)} &\colhead{(s)} &\colhead{}  %\\
%}
%\startdata
%XMM 	& 52,725	& 7.840 $\pm$ 0.004 	& \citet{Halpern2007} \\
%RXTE	&  53,216 & 7.82 $\pm$ 0.05 	& \citet{Markwardt2004} \\
%RXTE	&  54,682 & 7.839783 $\pm$ 0.000006 	& \citet{Markwardt2009} \\
%NuSTAR	&  58,346 & 7.84480 $\pm$ 0.00002 	& \citet{Shtykovsky2019} \\
%NICER	&  59,807 & 7.847089 $\pm$ 0.000015 	& \citet{Wolff2022} \\
%\enddata
%\tablecomments{ See Figure \ref{fig:pulse_history}
%}
%\label{table:pulse_history}
%\end{deluxetable}






